MixupExplainer: Generalizing Explanations for Graph Neural Networks with Data Augmentation

Graph Neural Networks (GNNs) have received increasing attention due to their ability to learn from graph-structured data. However, their predictions are often not interpretable. Post-hoc instance-level explanation methods have been proposed to understand GNN predictions. These methods seek to discover substructures that explain the prediction behavior of a trained GNN. In this paper, we shed light on the existence of the distribution shifting issue in existing methods, which affects explanation quality, particularly in applications on real-life datasets with tight decision boundaries. To address this issue, we introduce a generalized Graph Information Bottleneck (GIB) form that includes a label-independent graph variable, which is equivalent to the vanilla GIB. Driven by the generalized GIB, we propose a graph mixup method, MixupExplainer, with a theoretical guarantee to resolve the distribution shifting issue. We conduct extensive experiments on both synthetic and real-world datasets to validate the effectiveness of our proposed mixup approach over existing approaches. We also provide a detailed analysis of how our proposed approach alleviates the distribution shifting issue.

==> tabletexs/expl_auroc.tex <==
% \begin{table*}[t!]
%   \setlength{\tabcolsep}{4.5pt}
  
%   \caption{Explanation Faithfulness in terms of AUC on Edges}\label{tab:expl_auroc} 
%   \begin{tabular}{c|cccccc}
%     \hline
%                     & BA-Shapes                       & BA-Community                  & Tree-Circles                  & Tree-Grid                     & BA-2motifs                    & Mutag \\
%     \hline
%     GRAD            & $0.882$                         & $0.750$                       & $0.905$                       & $0.612$                       & $0.717$                       & $0.783$ \\
%     ATT             & $0.815$                         & $0.739$                       & $0.824$                       & $0.667$                       & $0.667$                       & $0.765$ \\
%     \hline
%     GNNExplainer    & $0.884_{\pm 0.002}$             & $0.682_{\pm 0.004}$           & $0.683_{\pm 0.009}$           & $0.379_{\pm 0.001}$           & $0.660_{\pm 0.006}$           & $0.539_{\pm 0.002}$ \\
%     + MixUp         & $0.890_{\pm 0.004}$             & $0.788_{\pm 0.006}$           & $0.690_{\pm 0.014}$           & $0.501_{\pm 0.003}$           & $0.869_{\pm 0.004}$           & $0.612_{\pm 0.043}$ \\
%     \hline
%     PGExplainer     & $0.999_{\pm 0.000}$             & $0.829_{\pm 0.040}$           & $0.762_{\pm 0.014}$           & $0.679_{\pm 0.008}$           & $0.679_{\pm 0.043}$           & $0.843_{\pm 0.084}$ \\
%     + MixUp         & $0.999_{\pm 0.001}$             & $0.955_{\pm 0.017}$           & $0.774_{\pm 0.004}$           & $0.712_{\pm 0.000}$           & $0.920_{\pm 0.031}$           & $0.871_{\pm 0.079}$ \\ 
%     \hline
%   \end{tabular}
%   \label{QEtable}
% \end{table*}
